Motzkin paths of bounded height with two forbidden contiguous subwords of length two

Motzkin excursions and meanders are revisited. This is considered in the context of forbidden patterns. Previous work by Asinowski, Banderier, Gittenberger, and Roitner is continued. Motzkin paths of bounded height are considered, leading to matrix equations and also to continued fractions. The enumeration is done by properly setting up bivariate generating functions which can be expanded using the kernel method.

==> DUHU.tex <==


\section{DU and HU are forbidden, A-new}
\begin{figure}[h]
	
	
	\begin{center}
		\begin{tikzpicture}[scale=1.5,main node/.style={circle,draw,font=\Large\bfseries}]
			
			
			
			\fill (0,0) circle (0.08cm);
			
			
			
			\foreach \x in {0,1,2,3,4,5,6,7}
			{
				\draw[thick, -latex] (\x,0) to  (\x+1,0);   
				      				\draw[thick, latex-,red] (\x,-1) [out=50,in=217]to  (\x+1,0);   
				      				%\draw[thick, latex-,red] (\x,-2) to  (\x+1,-1);   
				      				\draw[thick, latex-,red] (\x,-1) to  (\x+1,-1);   
				      								      			%	\draw[thick, latex-,red] (\x,-2) to  (\x+1,-2);   
					      				\draw[thick, -latex,red] (\x+1,-2) to  (\x,-1);   
				\node at  (\x+0.1,0.15){\tiny$\x$};
			}                        


			\foreach \x in {0,1,2,3,4,5,6,7,8}
{
		\draw[thick,-latex,blue ] (\x,-2)  ..  controls (\x-0.3,-0.3-2) and  (\x+0.3,-0.3-2) .. (\x,-2) ;	
	\draw[ thick,blue, latex-] (\x,-2)[in=-110,out=110]to  (\x,0);    
		\draw[ thick,blue, -latex] (\x,-1) to  (\x,-2);    

	
}                        
			
			\node at  (8+0.1,0.15){\tiny$8$};
			
			\foreach \x in {0,1,2,3,4,5,6,7,8}
			{%\node[main node] (\x) {\x};
				\draw (\x,-1) circle (0.05cm);
				\fill (\x,-1) circle (0.05cm);
				%     \node[circle,draw ] (c) at (\x,0){$\x$};
				\draw (\x,-2) circle (0.05cm);
				\fill (\x,-2) circle (0.05cm);
			}
		\foreach \x in {0,1,2,3,4,5,6,7,8}
		{%\node[main node] (\x) {\x};
			\draw (\x,0) circle (0.05cm);
			\fill (\x,0) circle (0.05cm);
		}
		\end{tikzpicture}
	\end{center}
	\caption{Graph (automaton) to recognize  Motzkin paths with forbidden subwords DU and HU.}
	\label{purpelDUHU}
\end{figure}
The recursion related to Figure \ref{purpelDUHU} are
\begin{align*}
	f_{i+1}&=zf_i+zh_i, \ f_0=1,\\
	g_i&=zf_{i+1}+zg_{i+1},\ i\ge0\\
	h_{i}&=zf_i+zg_{i}+zh_{i}
\end{align*}
and the system of functional equations is
\begin{align*}
	F(u)&=1+zuF(u)+zuH(u),\\
	G(u)&=\frac zu(G(u)-G(0))+\frac zu(H(u)-H(0)),\\
	H(u)&=zF(u)+zG(u)+z H(u).
\end{align*}
The ubiquitous denominator is $zu^2+(-1+z-z^2-z^3)u+z=z(u-r_1)(u-r_2)$ with
\begin{equation*}
r_1=\frac{1-z+z^2+z^3-W}{2z},\ r_2=\frac{1-z+z^2+z^3-W}{2z},\quad W=\sqrt{(1-z^4)(1-2z-z^2)}.
\end{equation*}
Dividing out the factor $u-r_1$ and simplifying, we end up with
\begin{equation*}
	F(u)=\frac{1}{1-ur_1},\ 	G(u)=\frac{(1-z)r_1-z}{z^2(1-ur_1)},\ 	H(u)=\frac{r_1-z}{z(1-ur_1)},\ 
S(u)=\frac{r_1-z}{z^2(1-ur_1)}.
\end{equation*}
We find
\begin{equation*}
S(0)=1+z+z^2+2z^3+4z^4+8z^5+16z^6+33z^7+69z^8+146z^9+312z^{10}+\cdots
\end{equation*}
which is A004149 in OEIS
and
\begin{equation*}
	S(1)=1+2z+4z^2+9z^3+20z^4+45z^5+102z^6+233z^7+535z^8+1234z^9+2857z^{10}+\cdots
\end{equation*}
1,2,4,9,20,45,102,233
which is A308435  in OEIS. Furthermore
\begin{equation*}
[u^j]S(u)=[u^j]\frac{r_1-z}{z^2(1-ur_1)}=\frac{r_1^{j+1}}{z^2}-\frac{r_1^{j}}{z}.
\end{equation*}
Since, before diving out the factor, we have
\begin{equation*}
	S(u) = \frac{\textsf{numerator}}{zu^2+(-1+z-z^2-z^3)u+z},
\end{equation*}
we get a recursion from it:
\begin{align*}
	zs_{j-2}+(-1+z-z^2-z^3)s_{j-1}+zs_j&=0,\ j\ge2,\\
(-1+z-z^3)s_0+zs_1&=z^2-1,
\end{align*}
which is in matrix form
{\scriptsize
\begin{equation*}
	\begin{pmatrix}
		-1+z-z^3& z& 0&\cdots  &0  \\
		z & -1+z-z^2-z^3&z& \cdots & 0 \\
		&		z & -1+z-z^2-z^3&z & 0 \\
		\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
		0 & 0 & \cdots&z &-1+z-z^2-z^3
	\end{pmatrix}
	\begin{pmatrix}
		s_0\\
		s_1\\
		s_2\\
		\vdots\\
		s_K
	\end{pmatrix}=
	\begin{pmatrix}
		z^2-1\\
		0\\
		0\\
		\vdots\\
		0
	\end{pmatrix}
\end{equation*}}
The usual determinant is
\begin{equation*}
	\mD_{K}=(-1+z-z^2-z^3)\mD_{K-1}-z^2\mD_{K-2}=\frac{(-z)^{K+1}}{W}(r_1^{K+1}-r_2^{K+1}).
\end{equation*}
With $t_K=\mD_{K-1}/\mD_{K}$ and $\tau_K=-z^2t_K$,
\begin{equation*}
	t_K=\frac{1}{-1+z-z^2-z^3-z^2t_{K-1}}\ \Longrightarrow \ \tau_K=\frac{z^2}{1-z+z^2+z^3-\tau_{K-1}},\ \tau_0=0.
\end{equation*}
Since $\phi_K=1$ for all $K$, we concentrate on the remaining two:
{\scriptsize
	\begin{equation*}
		\begin{pmatrix}
			-1+2z-z^2+z^4& z(1-z)& 0&\cdots  &0  \\
			z & -1+z-z^2-z^3&z& \cdots & 0 \\
			&		z & -1+z-z^2-z^3&z & 0 \\
			\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
			0 & 0 & \cdots&z &-1+z-z^2-z^3
		\end{pmatrix}
		\begin{pmatrix}
			g_0\\
			g_1\\
			g_2\\
			\vdots\\
			g_K
		\end{pmatrix}=
		\begin{pmatrix}
			-z^3\\
			0\\
			0\\
			\vdots\\
			0
		\end{pmatrix}
\end{equation*}}
{\scriptsize
	\begin{equation*}
		\begin{pmatrix}
			-1+z-z^3& z& 0&\cdots  &0  \\
			z & -1+z-z^2-z^3&z& \cdots & 0 \\
			&		z & -1+z-z^2-z^3&z & 0 \\
			\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
			0 & 0 & \cdots&z &-1+z-z^2-z^3
		\end{pmatrix}
		\begin{pmatrix}
			h_0\\
			h_1\\
			h_2\\
			\vdots\\
			h_K
		\end{pmatrix}=
		\begin{pmatrix}
			z(z^2-1)\\
			0\\
			0\\
			\vdots\\
			0
		\end{pmatrix}
\end{equation*}}



From this, we can express the solutions (return to the $x$-axis) in continued fraction form
\begin{align*}
	s_0=\sigma_{K+1}&=\frac{(z^2-1)\mD_{K}}{	(-1+z-z^3)\mD_{K}-z^2\mD_{K-1}}
	=\frac{(z^2-1)}{	(-1+z-z^3)-z^2t_{K}}\\&=\frac{1-z^2}{	1-z+z^3-\tau_{K}},\	\ \sigma_0=\frac1{1-z},\\
	g_0=\gamma_{K+1}&=\frac{-z^3\mD_{K}}{(-1+2z-z^2+z^4)\mD_{K}-z^2(1-z)\mD_{K-1}}\\&
	=\frac{z^3}{1-2z+z^2-z^4-(1-z)\tau_{K}}	,\  \gamma_0=0,\\
	h_0=\eta_{K+1}&=\frac{z(z^2-1)\mD_{K}}{(-1+z-z^3)\mD_{K}-z^2\mD_{K-1}}\\&=
	\frac{z(z^2-1)}{(-1+z-z^3)-z^2t_{K}}=\frac{z(1-z^2)}{1-z+z^3-\tau_{K}},\ \eta_0=\frac{z}{1-z}.
\end{align*}



==> UDDH.tex <==


\section{UD and DH are forbidden, A023431}
\begin{figure}[h]
	
	
	\begin{center}
		\begin{tikzpicture}[scale=1.5,main node/.style={circle,draw,font=\Large\bfseries}]
			
			
			
			\fill (0,0) circle (0.08cm);
			
			
			
			\foreach \x in {0,1,2,3,4,5,6,7}
			{
				\draw[thick, -latex] (\x,0) to  (\x+1,0);   
				      				\draw[thick, -latex] (\x,-1) [out=50,in=217]to  (\x+1,0);   
				      				\draw[thick, latex-,red] (\x,-2) to  (\x+1,-1);   
				      								      				\draw[thick, latex-,red] (\x,-2) to  (\x+1,-2);   
					      				\draw[thick, -latex] (\x,-2) to  (\x+1,0);   
				\node at  (\x+0.1,0.15){\tiny$\x$};
			}                        




			\foreach \x in {0,1,2,3,4,5,6,7,8}
{
		\draw[thick,-latex,blue ] (\x,-1)  ..  controls (\x-0.1,-0.3-1) and  (\x+0.3,-0.2-1) .. (\x,-1) ;	
	\draw[ thick,blue, latex-] (\x,-1)to  (\x,0);    

	
}                        
			
			\node at  (8+0.1,0.15){\tiny$8$};
			
			\foreach \x in {0,1,2,3,4,5,6,7,8}
			{%\node[main node] (\x) {\x};
				\draw (\x,-1) circle (0.05cm);
				\fill (\x,-1) circle (0.05cm);
				%     \node[circle,draw ] (c) at (\x,0){$\x$};
				\draw (\x,-2) circle (0.05cm);
				\fill (\x,-2) circle (0.05cm);
			}
		\foreach \x in {0,1,2,3,4,5,6,7,8}
		{%\node[main node] (\x) {\x};
			\draw (\x,0) circle (0.05cm);
			\fill (\x,0) circle (0.05cm);
		}
		\end{tikzpicture}
	\end{center}
	\caption{Graph (automaton) to recognize  Motzkin paths with forbidden subwords UD and HH.}
	\label{purpelUDHU}
\end{figure}
The recursion related to Figure \ref{purpelUDHU} are
\begin{align*}
	f_{i+1}&=zf_i+zg_i+zh_i, \ f_0=1,\\
	g_i&=zf_i+zg_i,\ i\ge0\\
	h_{i}&=zg_{i+1}+zh_{i+1}
\end{align*}
and the system of functional equations is
\begin{align*}
	F(u)&=1+zuF(u)+zuG(u)+zuH(u),\\
	G(u)&=zF(u)+zG(u)+zH(u),\\
	H(u)&=\frac zu(G(u)-G(0))+\frac zu(H(u)-H(0)).
\end{align*}
The ubiquitous denominator is $zu^2+(z-1)u+z^2=z(u-r_1)(u-r_2)$ with
\begin{equation*}
r_1=\frac{1-z-W}{2z},\ r_2=\frac{1-z+W}{2z},\quad W=\sqrt{1-2z+z^2-4z^3}.
\end{equation*}
Dividing out the factor $u-r_1$ and simplifying, we end up with
\begin{equation*}
	F(u)=\frac{ur_1}{z-ur_1},\ G(u)=1+\frac{r_1}{z-ur_1},\ H(u)=\frac{(1-z)r_1-z^2}{z(z-ur_1)},\ S(u)=\frac{r_1}{z(z-ur_1)}.
\end{equation*}
We find
\begin{equation*}
S(0)=1+z+z^2+2z^3+4z^4+7z^5+13z^6+26z^7+52z^8+104z^9+212z^{10}+\cdots
\end{equation*}
which is A023431 in OEIS
and
\begin{equation*}
	S(1)=1+2z+4z^2+9z^3+21z^4+49z^5+115z^6+272z^7+646z^8+1538z^9+3670z^{10}+\cdots
\end{equation*}
which is not in OEIS. Furthermore
\begin{equation*}
[u^j]S(u)=[u^j]\frac{r_1}{z(z-ur_1)}=[u^j]\frac{r_1}{z^2(1-\frac{ur_1}{z})}=\frac1z\Big(\frac{r_1}{z}\Big)^{j+1}
\end{equation*}

Since, before diving out the factor, we have
\begin{equation*}
	S(u) = \frac{-u-z-uz^2G(0)+zG(0)}{-u+zu^2+z^2+zu},
\end{equation*}
we get a recursion from it:
\begin{align*}
	zs_{j-2}+(z-1)s_{j-1}+z^2s_j&=0,\ j\ge2\\
	(z-1)s_0+z^2s_1&=-1,
\end{align*}
which is in matrix form
\begin{equation*}
	\begin{pmatrix}
		z-1& z^2& 0&\cdots  &0  \\
		z & z-1 &z^2& \cdots & 0 \\
		&		z & z-1 &z^2 & 0 \\
		\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
		0 & 0 & \cdots&z &z-1
	\end{pmatrix}
	\begin{pmatrix}
		s_0\\
		s_1\\
		s_2\\
		\vdots\\
		s_K
	\end{pmatrix}=
	\begin{pmatrix}
		-1\\
		0\\
		0\\
		\vdots\\
		0
	\end{pmatrix}
\end{equation*}
The usual determinant is
\begin{equation*}
	\mD_{K}=(z-1)\mD_{K-1}-z^3\mD_{K-2}=\frac{(-z)^{K+1}}{W}(r_1^{K+1}-r_2^{K+1}).
\end{equation*}
With $t_K=\mD_{K-1}/\mD_{K}$ and $\tau_K=-z^3t_K$
\begin{equation*}
	t_K=\frac{1}{z-1-z^3t_{K-1}}\ \Longrightarrow \ \tau_K=\frac{z^3}{1-z-\tau_{K-1}},\ \tau_0=0
\end{equation*}
\begin{equation*}
	\begin{pmatrix}
		z-1& z^2& 0&\cdots  &0  \\
		z & z-1 &z^2& \cdots & 0 \\
		&		z & z-1 &z^2 & 0 \\
		\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
		0 & 0 & \cdots&z &z-1
	\end{pmatrix}
	\begin{pmatrix}
		g_0\\
		g_1\\
		g_2\\
		\vdots\\
		g_K
	\end{pmatrix}=
	\begin{pmatrix}
		-1\\
		z\\
		0\\
		\vdots\\
		0
	\end{pmatrix}
\end{equation*}
\begin{equation*}
	\begin{pmatrix}
		-1+2z-z^2+z^3& z^2(1-z)& 0&\cdots  &0  \\
		z & z-1 &z^2& \cdots & 0 \\
		&		z & z-1 &z^2 & 0 \\
		\vdots  & \ddots  & \ddots & \ddots  & \vdots\\
		0 & 0 & \cdots&z &z-1
	\end{pmatrix}
	\begin{pmatrix}
		h_0\\
		h_1\\
		h_2\\
		\vdots\\
		h_K
	\end{pmatrix}=
	\begin{pmatrix}
		-z^3\\
		0\\
		0\\
		\vdots\\
		0
	\end{pmatrix}
\end{equation*}
From this, we can express the solutions (return to the $x$-axis) in continued fraction form
\begin{align*}
	s_0=\sigma_{K+1}&=\frac{-\mD_{K}}{(z-1)\mD_{K}-z^3\mD_{K-1}}=\frac{1}{1-z+z^3t_{H}}=\frac{1}{1-z-\tau_{H}},\ \sigma_0=\frac1{1-z},\\
	g_0=\gamma_{K+1}&=\frac{-\mD_{K}-z^3\mD_{K-1}}{(z-1)\mD_{K}-z^3\mD_{K-1}}
	=\frac{-1-z^3t_{K}}{z-1-z^3t_{K}}=1+\frac{z}{1-z-\tau_K},\  \gamma_0=\frac1{1-z},\\
	h_0=\eta_{K+1}&=\frac{-z^3\mD_{K}}{(-1+2z-z^2+z^3)\mD_{K}-z^3(1-z)\mD_{K-1}}=
	\frac{z^3}{1-2z+z^2-z^3-(1-z)\tau_{K}},\ \eta_0=0.
\end{align*}


